Ambitwistor Yang-Mills Theory Revisited

Inspired by the Movshev-Mason-Skinner Cauchy-Riemann (CR) ambitwistor approach, we provide a rigorous yet elementary construction of a twisted CR holomorphic Chern-Simons action on CR ambitwistor space for maximally supersymmetric Yang-Mills theory on four-dimensional Euclidean space. The key ingredient in our discussion is the homotopy algebraic perspective on perturbative quantum field theory. Using this technology, we show that both theories are semi-classically equivalent, that is, we construct a quasi-isomorphism between the cyclic $L_\infty$-algebras governing both field theories. This confirms a conjecture from the literature. Furthermore, we also show that the Yang-Mills action is obtained by integrating out an infinite tower of auxiliary fields in the Chern-Simons action, that is, the two theories are related by homotopy transfer. Given its simplicity, this Chern-Simons action should form a fruitful starting point for analysing perturbative properties of Yang-Mills theory.

==> lib/characters.tex <==
\newcommand{\makecommand}[3]{%
	\foreach \i in #3 {%
    	\expandafter\xdef\csname #1\i\endcsname{{\noexpand#2{\unexpanded\expandafter{\i}}}}%
  	}%
}

%
% Characters
%

\newcommand{\latinalphabet}{A,a,B,b,C,c,d,D,E,e,F,f,G,g,H,h,I,i,J,j,K,k,L,l,M,m,N,n,O,o,P,p,Q,q,R,r,S,s,T,t,U,u,V,v,W,w,X,x,Y,y,Z,z}
\newcommand{\Latinalphabet}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makecommand{I}{\mathbbm}{\latinalphabet}
\makecommand{bf}{\mathbf}{\latinalphabet}
\makecommand{bm}{\bm}{\latinalphabet}
\makecommand{ca}{\mathcal}{\Latinalphabet}
\makecommand{fr}{\mathfrak}{\latinalphabet}
\makecommand{rm}{\mathrm}{\latinalphabet}
\makecommand{sf}{\mathsf}{\latinalphabet}
\makecommand{sc}{\mathscr}{\latinalphabet}
\makecommand{tt}{\mathtt}{\latinalphabet}

\makecommand{bar}{\bar}{\latinalphabet}
\makecommand{dot}{\dot}{\latinalphabet}

\newcommand{\eps}{\varepsilon}

%
% Lie groups and algebras
%

\makecommand{sf}{\mathsf}{{GL,SL,O,SO,OSp,U,SU,Sp,Spin}}
\makecommand{fr}{\mathfrak}{{Lie,gl,sl,o,so,osp,u,su,sp,spin}}

%
% Categories, operads, etc.
%

\makecommand{Cat}{\mathsf}{{Ass,Cat,Com,DiffCat,End,Fun,Gr,GradSMod,GradVect,Grp,Lie,Mfd,Oper,poSet,Schur,SMod,Set,SMfd,sGrp,sMfd,sSet,sSMfd,SurSub,Top,Vect,VectBun}}

\makecommand{sf}{\mathsf}{{CE,Ch,Der,Diag,End,Hom,hom,inthom,Jet,Kan,TDiff}}

\newcommand{\opEnd}{{{\caE}nd}}
\newcommand{\OpEnd}{{{\scE}\!nd}}
\newcommand{\opCom}{{{\caC}om}}
\newcommand{\OpCom}{{{\scC}\!om}}
\newcommand{\opAss}{{{\caA}ss}}
\newcommand{\OpAss}{{{\scA}\!ss}}
\newcommand{\opLie}{{{\caL}ie}}
\newcommand{\OpLie}{{{\scL}\!ie}}
\newcommand{\opGer}{{{\caG}er}}
\newcommand{\OpGer}{{{\scG}\!er}}
\newcommand{\opBV}{{{\caB\caV}}}
\newcommand{\OpBV}{{{\scB\scV}}}
\newcommand{\opqBV}{{q{\caB\caV}}}
\newcommand{\OpqBV}{{q{\scB\scV}}}
\newcommand{\opDual}{{{\caD}ual}}
\newcommand{\OpDual}{{{\scD}\!ual}}
\newcommand{\opGam}{{{\caG}am}}
\newcommand{\OpGam}{{{\caG}\!am}}
\newcommand{\opHom}{{{\caH}om}}
\newcommand{\OpHom}{{{\caH}\!om}}

==> lib/commands.tex <==
%
% Arrows
%

\newcommand{\multirightarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\newcommand{\multileftarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\renewcommand{\twoheadrightarrow}{\mathrel{\mathrlap{\rightarrow}\mkern.5mu\rightarrow}}
\DeclareRobustCommand\longtwoheadrightarrow{\relbar\joinrel\twoheadrightarrow}
\renewcommand{\twoheadleftarrow}{\mathrel{\mathrlap{\leftarrow}\mkern.5mu\leftarrow}}
\DeclareRobustCommand\longtwoheadleftarrow{\twoheadleftarrow\joinrel\relbar}

%
% Derivatives
%

\newcommand{\dder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\mathrm{d}}{\mathrm{d} #2}%
	}{%
		\frac{\mathrm{d} #1}{\mathrm{d} #2}%
	}%
}
\newcommand{\parder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\partial}{\partial #2}%
	}{%
		\frac{\partial #1}{\partial #2}%
	}%
}
\newcommand{\delder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\delta}{\delta #2}%
	}{%
		\frac{\delta #1}{\delta #2}%
	}%
}

%
% Inner products
%

\newcommand{\inner}[2]{\langle#1,#2\rangle}
\newcommand{\innerLarge}[2]{\left\langle#1,#2\right\rangle}

%
% Vectors
%

\newcommand{\colvec}[1]{%
    \begingroup
        \newcommand\listcontent{}
        \def\do##1{\appto\listcontent{##1\\}}
        \expandafter\docsvlist\expandafter{#1}
        \begin{pmatrix}
            \listcontent
        \end{pmatrix}
    \endgroup
}

%
% Integrals
%

\DeclareMathOperator*{\sumint}{%
\mathchoice%
	{\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}

\DeclareMathOperator*{\cpv}{\setbox0=\hbox{$\int$}\int\hskip-\wd0{}\hskip-\wd0{~-~}} % Cauchy principal value

%
% Miscellaneous
%

\newcommand\acton{\mathbin\vartriangleright} % action
\DeclareMathOperator{\Ad}{Ad} % adjoint map
\DeclareMathOperator{\ad}{ad} % adjoint map
\DeclareMathSymbol{\antishriek}{\mathord}{operators}{'74} %antishriek
\DeclareMathOperator{\coker}{coker} % cokernel
\DeclareMathOperator{\diag}{diag} % diagonal matrix
\DeclareMathOperator{\lvac}{\langle 0|} % vacuum
\DeclareMathOperator{\id}{\mathrm{id}} % identity
\DeclareMathOperator{\sfid}{\mathsf{id}} % identity
\DeclareMathOperator{\im}{im} % image
\newcommand{\normal}[1]{\mathop{:\mathrel{#1}:}} % normal ordering
\DeclareMathOperator{\pr}{\mathsf{pr}} % projection
\newcommand{\spacer}[1]{\vrule width0pt height0pt depth#1\relax}
\DeclareMathOperator{\spn}{span} % span
\DeclareMathOperator{\str}{str} % super trace
\newcommand{\tocut}[1]{{\color{green} #1 }}
\newcommand{\todo}[1]{{\color{red} #1 }}
\DeclareMathOperator{\tr}{tr} % trace
\DeclareMathOperator{\rvac}{|0\rangle} % vacuum
%\newcommand{\uline}[1]{\ul{\itshape #1}}
\newcommand{\uline}[1]{\ul{\emph{#1}}}
\DeclareMathOperator{\unit}{\mathbbm{1}} % unit matrix
\DeclareMathOperator{\lap}{\mathop\Delta\nolimits} % Laplacian
\DeclareMathOperator{\wave}{{\mathop\oldsquare\nolimits}} % adjust sup/subscripts for the d'Alembertian
\DeclareMathOperator{\intprod}{\mathbin{\raisebox{\depth}{\scalebox{1}[-1]{$\lnot$}}}} % interior product

%
% Prepositions
%

\newcommand{\efor}{{~~~\mbox{for}~~~}}
\newcommand{\eforall}{{~~~\mbox{for all}~~~}}
\newcommand{\eand}{{~~~\mbox{and}~~~}}
\newcommand{\eon}{{~~\mbox{on}~~}}
\newcommand{\eor}{{~~~\mbox{or}~~~}}  		
\newcommand{\ewith}{{~~~\mbox{with}~~~}}
\newcommand{\eelse}{{~~~\mbox{else}~~~}}

%
% Young diagrams
%

\newcommand{\tyng}[1]{\hbox{\tiny$\yng #1$}} % small Young diagram
\newcommand{\tyoung}[1]{\hbox{\tiny$\young #1$}} % small Young diagram


==> lib/hyphenation.tex <==
\hyphenation{mani-folds mani-fold opera-tor bet-ween}
